Multi-Task Learning For Reduced Popularity Bias In Multi-Territory Video Recommendations

Various data imbalances that naturally arise in a multi-territory personalized recommender system can lead to a significant item bias for globally prevalent items. A locally popular item can be overshadowed by a globally prevalent item. Moreover, users' viewership patterns/statistics can drastically change from one geographic location to another which may suggest to learn specific user embeddings. In this paper, we propose a multi-task learning (MTL) technique, along with an adaptive upsampling method to reduce popularity bias in multi-territory recommendations. Our proposed framework is designed to enrich training examples with active users representation through upsampling, and capable of learning geographic-based user embeddings by leveraging MTL. Through experiments, we demonstrate the effectiveness of our framework in multiple territories compared to a baseline not incorporating our proposed techniques.~Noticeably, we show improved relative gain of up to $65.27\%$ in PR-AUC metric. A case study is presented to demonstrate the advantages of our methods in attenuating the popularity bias of global items.

==> Sections_Belhassen/Approach_v0.tex <==
\section{Approach}

==> Sections_Belhassen/Conclusion_v0.tex <==
\section{Conclusion}

==> Sections_Belhassen/Experiments_v0.tex <==
\section{Experiments}

==> Sections_Belhassen/Intro_v0.tex <==
\section{Introduction}

==> Sections_Belhassen/Problem_Statement_v0.tex <==
\section*{Customer Problem Statement}

==> Sections_Belhassen/Related_Work_v0.tex <==
\section{Related Work}

==> Sections_Farnoosh/Abstract.tex <==
Various data imbalances that naturally arise in a multi-territory personalized recommender system can lead to a significant item bias for globally prevalent items. A locally popular item can be overshadowed by a globally prevalent item. At the same time, the viewership patterns are expected to change from one territory to another across the globe. Training and maintaining models for each territory across the globe can be prohibitive and redundant.~It would be ideal to learn some shared representations across territories and then localise them using transfer learning. In this paper, we present two techniques, adaptive upsampling and multi-task learning (MTL), that we have developed to mitigate geographical item popularity bias and to better deal with the differences in viewing patterns across territories. Through a series of experiments, we demonstrate the effectiveness of the proposed techniques, where we show improved relative gain of upto 65 \% in PR-AUC metric against the baseline model when evaluated in multiple territories. Through a case study, we also demonstrate the advantages of the proposed techniques in attenuating the popularity bias of global titles.
% Although MTL is a widely studied technique, this is a novel application of MTL to address geographical popularity bias. We are currently implementing this fairness-enhanced model in production.

==> Sections_Farnoosh/Introduction.tex <==
\section{Introduction}
In modern streaming services such as YouTube, Prime Video, Netflix and etc., recommender systems (RS) have become the cornerstone of user engagement by helping the users find relevant contents~\cite{amatriain2015recommender,berkovsky2017recommend}. ML-based RS are typically trained in a supervised way using the logs of previous user-item interactions as explicit or implicit feedback of user’s interest ~\cite{gomez2015netflix,cheng2016wide}. For RS with wide geographical coverage across multiple countries such as the Amazon Prime Video, theoretically-speaking, one may design multiple ML models which are trained on and are specialized at making recommendations for different regions. Maintaining such a multi-model is challenging from the ML operational perspective. It is therefore, highly preferable for a large-scale recommendation system to create one global model that can learn to make useful recommendations across different geographical regions. 


One common challenge for successfully training ML-based RS is the various imbalances that naturally occur in the user-item interaction training data~\cite{chen2020bias,gomez2020characterizing}. In this work, we are particularly concerned with the data imbalances that exist across different geographical sections of a global RS for Amazon Prime Video with worldwide coverage. This data imbalance can occur in any multi-territory setting. For instance, one video title can be the 10’th popular title in one territory but still have much more user interaction history than the most popular video title in other territories. In addition, user interaction history data of a video title that is only streamed in one specific territory (i.e., a local item) can be significantly smaller than that of a video title that is streamed in multiple territories (i.e., a global item), even though the local item/title is much more popular in that specific territory. If these imbalances are not properly handled, the global RS will inevitably suppress the locally popular items at the expense of globally present items. In other words, a single global model would suffer from a popularity bias towards globally present items. 

\input{Sections_Phanideep/Introduction_paras}

% We address the data imbalance issue in our system by means of a data-centric and a model-centric approach, which are our key contributions, as follows:  

% (1) A data upsampling strategy in order to capture the customer embeddings of active customers.This additional filter helps us to gather more training examples for a title only if it is truly popular. At the same time, it would also increase the training examples for local popular titles. (2) A Multi Task Learning(MTL) approach which we will describe in section \ref{subsec:MTL two tower model}. With this MTL approach, the performance of the majority of territories improves and we de-risk and reduce the global popularity bias effect. In addition, small territories will also benefit from larger territories. We will discuss the architecture of our proposed model in detail in section.

Our baseline model architecture consists of a two-tower Neural Network (NN) model ~\cite{huang2013learning} (one tower for user and one title) which learns propensity score for a user’s first time content discovery by leveraging learned representation of user and title embeddings which are vended by an upstream representation learning feature store. The exact details are described in section~\ref{subsec:input_embeddings}.
%
Through a set of experiments, we compared our baseline recommendation system to a model that leverages the MTL approach and upsampling strategy. Our experimental results demonstrate the advantage of our proposed model which improved the PR-AUC of the majority territories significantly and also helped to reduce the popularity bias toward global titles.
\label{section:introduction}


==> Sections_Farnoosh/Problem_Statement.tex <==
\section*{Customer Problem Statement}

Once we deploy our worldwide model, this work will have a direct impact on our prime video customers. Our customers will benefit from more accurate recommendations for items that are popular in their country but not necessarily prevalent globally as demonstrated in our offline experiments. 
Our proposed technique will improve the recommendation accuracy for the majority of items and territories and we believe it will lead to an overall improved customer engagement and satisfaction. It should be noted, however, that popularity bias may not be fully solved for all possible territory and item combinations.~As a result of this bias, our customers might receive some irrelevant recommendations which may not be an ideal experience. Our team will measure customer engagement signals both during A/B testing and post deployment. 

==> Sections_Farnoosh/data_stats.tex <==
Our training data consists of 6MM customers. 
We grouped more than 200 territories into 4 groups. This criteria groups geographically closer territories together, that can have similar viewing patterns. At the same time, there is also a relatively good balance of major and minor territories in each group. Table below shows the number of territories per each group. 


\begin{table}[h]
\label{table: Groups-territory}
\begin{tabular}{ p{1.0 cm} p{1.0 cm} p{1.0 cm} p{1.0 cm}}
    \toprule
   Group1 & Group2 & Group3  & Group4  \\
    \midrule
    \multirow{1}{*} 31 & 80&80&38 \\
    \bottomrule
\end{tabular}
\end{table}

==> Sections_Phanideep/Introduction_paras.tex <==
Popularity bias arising from the data imbalance decreases the fairness of the recommendations~\cite{abdollahpouri2019unfairness,abdollahpouri2020multi}, specifically for the titles local to a certain country. And the bias would only amplify in a closed feedback setting~\cite{chen2020bias,zhu2021popularity}, where the titles present in a lot of territories are always ranked higher and the gap between the global and local titles would either remain the same or increase. To prevent the model from overfitting on the global titles and to improve the fairness of local titles, we propose the use of Hard Parameter Sharing based Multi Task Learning (MTL)~\cite{caruana1993multitask} approach. MTL has strong regularisation properties~\cite{ruder2017overview,baxter1997bayesian} that improves the generalisation power of the model by preventing overfitting on global titles. At the same time, MTL learns shared representations that can be used by countries with less data allowing the transfer of knowledge from countries with large data. 

Rebalancing and regularisation are among the frequent techniques used for solving the unfairness issue arising from the data imbalance~\cite{chen2020bias} in the field of recommendation. We address the popularity bias issue in our system by means of a data-centric and a model-centric approach, which are our key contributions, as follows: (1) A data upsampling strategy based on active users criteria to enrich the training data with more number of informative examples to learn from. (2) A Multi Task Learning (MTL) approach to learn the refined user representations at a territory group level to deal with the distributional differences of viewership patterns across different territories. (3) Through a case study, we show how MTL reduces the popularity bias of global titles by learning group-specific parameters from the conditional distributions at a territory group level.

% \textcolor{orange}{to filter out the deemed not popular positive examples from the training data?}
